SNAP: Stateful Network-Wide Abstractions for Packet Processing

Early programming languages for software-defined networking (SDN) were built on top of the simple match-action paradigm offered by OpenFlow 1.0. However, emerging hardware and software switches offer much more sophisticated support for persistent state in the data plane, without involving a central controller. Nevertheless, managing stateful, distributed systems efficiently and correctly is known to be one of the most challenging programming problems. To simplify this new SDN problem, we introduce SNAP. SNAP offers a simpler "centralized" stateful programming model, by allowing programmers to develop programs on top of one big switch rather than many. These programs may contain reads and writes to global, persistent arrays, and as a result, programmers can implement a broad range of applications, from stateful firewalls to fine-grained traffic monitoring. The SNAP compiler relieves programmers of having to worry about how to distribute, place, and optimize access to these stateful arrays by doing it all for them. More specifically, the compiler discovers read/write dependencies between arrays and translates one-big-switch programs into an efficient internal representation based on a novel variant of binary decision diagrams. This internal representation is used to construct a mixed-integer linear program, which jointly optimizes the placement of state and the routing of traffic across the underlying physical topology. We have implemented a prototype compiler and applied it to about 20 SNAP programs over various topologies to demonstrate our techniques' scalability.

==> background.tex <==
\section{Background on NetKAT}\label{sec:background}
This section provides some background on NetKAT~\cite{NetKAT}, a domain-specific language for specifying and reasoning about networks, from which \Lang borrows its basis from.
To start with the reasons for choosing NetKAT; as mentioned earlier, \Lang is expected to express a large set of policies, each involves a set of packet tests and transformations. Therefore some mechanism that support combining these policies into a single one is required. NetKAT offers primitives for \emph{parallel and sequential compositions}, therefore it is a natural choice for this task.
NetKAT has attracted a lot of academic attention over the last couple of years, such as the design of an efficient compiler~\cite{FastNetKATCompiler} whose constructs we have adopted.  

\textbf{Expressions} --- NetKAT is designed to express the forwarding policy based on packet's location and information in its headers. 
A NetKAT expression can be thought of as a function that receives a packet and outputs a set of zero or more packets. 
There are two main types of expressions, predicates that act as filters) and policies that include predicates and also support actions such as field modification and packet duplication. 


\textbf{Filters} ---
include a set of primitives: the identity (1) outputs the singleton set of the input packet, drop (0) returns the empty set, and test ($f = v$), which acts like identity when the value of $f$ field in the input packet is $v$ and 
returns the empty set otherwise;  
as well as a set of operators for combining them; negation ($\neg$), conjunction ($;$) and disjunction ($+$). 

\textbf{Policies} ---
include predicates and a primitive action for field modification (\modify{f}{v}). Fields include a set of common header fields as well as two additional ones that indicate the packet location: switch and port. For example the following policy \code{sw=1;\modify{pt}{2}} means filter out all packets but those at switch 1 and send them to its port 2. Policies also include operators for combining
policies --- parallel composition ($+$) and sequential composition ($;$).

\textbf{Parallel composition} --- $(p+q)$ provides the programmer an abstraction that allows combining two policies without specifying an order of execution. $(p+q)$ executes $p$ and $q$ separately and outputs the union of 
the results. In a basic example where there is a single input packet, $p$ is leaves the packet unchanged and $q$ modifies a field, $(p + q)$ produces two packets in its output. A more illustrative example may be of performing multicast of a packet to seven different output ports. This is accomplished by parallel composition of seven different policies, each modifies the out port of the packet to a different one. 

\textbf{Sequential composition} --- $(p;q)$, takes the output of $p$ and uses it as input to $q$. If $p$ generates multiple packets, $q$ is executed
on each separately and the union of the results are returned.
$p*$ may be thought as a sequential composition of $p$ with itself for zero or more times. It is usually used to express packet traversal over the network topology. 

Figure~\ref{fig:syntax} describes \Lang 's syntax, which provides the general notion of NetKAT's syntax except for its missing iteration operator (since \Lang uses a One Big Switch abstraction that abstracts topology, thus iteration is not needed) and excluding \Lang 's additions, which are marked as bold. 

